Smoothness and effective regularizations in learned embeddings for shape matching

Many innovative applications require establishing correspondences among 3D geometric objects. However, the countless possible deformations of smooth surfaces make shape matching a challenging task. Finding an embedding to represent the different shapes in high-dimensional space where the matching is easier to solve is a well-trodden path that has given many outstanding solutions. Recently, a new trend has shown advantages in learning such representations. This novel idea motivated us to investigate which properties differentiate these data-driven embeddings and which ones promote state-of-the-art results. In this study, we analyze, for the first time, properties that arise in data-driven learned embedding and their relation to the shape-matching task. Our discoveries highlight the close link between matching and smoothness, which naturally emerge from training. Also, we demonstrate the relation between the orthogonality of the embedding and the bijectivity of the correspondence. Our experiments show exciting results, overcoming well-established alternatives and shedding a different light on relevant contexts and properties for learned embeddings.

==> sections/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Finding a convenient representation for deformable $3$D objects is a central research question which has attracted attention for decades \cite{torgerson1952multidimensional,bronstein2006generalized,wu20153d}. 
From a historical perspective, the bulk of the work has gone into the construction of shape embeddings into a high-dimensional space, where complex (e.g. non-rigid) transformations are factored out or translated to simpler transformations.

For example, a general procedure is to embed the intrinsic geometry of a 3D shape into a higher-dimensional space where Euclidean distances approximate the intrinsic metric of the object (multidimensional scaling)~\cite{torgerson1952multidimensional}. The convenience of such an approach is clear, as we are naturally inclined to work with extrinsic distances (lengths of straight lines in Euclidean space) instead of intrinsic ones (lengths of curved paths on a surface).

\begin{figure*}
\centering
			\begin{overpic}[trim=0cm 0cm 0cm 0cm,clip, width=0.80\linewidth]{./figures/pair1_lbo.png}
			\put(15,0){$\M$}
			\put(40,0){Our}
			\put(75,0){$GFM_{DN}$}
			\end{overpic}
\caption{\label{fig:teaser} An example of extreme non-isometric matching. The left shape is a statue from \cite{scantheworld}, the second is a gorilla from \cite{TOSCA}.}
\end{figure*}

Similarly, the eigenfunctions of the Laplace-Beltrami Operator (LBO) played a prominent role in deformable shape representation. Their theoretical properties (i.e., their analogy with the Fourier basis, together with their natural ordering, orthogonality, and smoothness) make them convenient for several applications including, but not limited to, surface fairing, function analysis, segmentation, and shape matching \cite{field1988laplacian,reuter2009discrete,ovsjanikov2012functional}. The latter, in particular, is among the most challenging tasks in 3D geometry processing to date. A recent approach to tackle this task is embodied in the framework of functional map \cite{ovsjanikov2012functional}, which casts the point-to-point correspondence problem as one of recovering a linear map among functional spaces defined over the input surfaces. The estimation of the correspondence via functional maps can be seen as seeking an alignment between two high-dimensional point clouds \cite{ovsjanikov2012functional,cpd,fspm} given by the underlying shape via the Laplacian eigenfunctions. While this framework does not rely on any particular choice of bases, the LBO eigenbasis constitutes a natural choice due to its optimality for representing smooth functions~\cite{Aflalo15}. Further, while many variants have been proposed \cite{choukroun2016hamiltonian,LMH,CMH,melzi2019sparse}, the literature is almost unanimous in adopting the LBO eigenbasis as the {\em de facto} standard for shape matching. 
Along this line of thought, \cite{LIE2020} proposed to {\em learn} an alternative embedding. It offers an introduction to this framework and provides promising results, but tackling only sparse point clouds (where LBO approximation is less stable) requires large datasets for training. \cite{LIE2020} only scratched the surface of this direction without offering any analysis of the learned basis. This lack is also a consequence of addressing a domain in which no good alternatives are known.

Concerning \cite{LIE2020}, we instantiate the method to work on meshes providing a more coherent comparison with LBO. For this reason, we adopt a state-of-the-art feature extractor for surfaces \cite{sharp2020diffusion}. This approach casts our work directly in the domain where LBO eigenfunctions have played the lion's share for decades. \rickn{Also, no previous studies have questioned the impact and relevance of orthogonality and smoothness.} We investigate such properties for the first time, \rickn{juxtaposing theoretical and empirical evidence to the common intuition.} 
%Our work motivates us to 
We foster this research direction in the meshes case and, exploiting the prior given by the surface (connectivity information), we prove that our method can deal with limited training samples.

The new data-driven embedding provides better performance and generalization than LBO eigenfunctions. Moreover, it enables us to investigate \simone{the influence of the different} properties, which ones have contributed to the LBO eigenfunctions success, and which ones need to be relaxed.

We learn and analyze embeddings in settings in which LBO is extremely powerful, like nearly-isometric matching; the community considers such a problem almost saturated, but we show that further improvement is possible. We also tackle open problems with a critical applicative impact (i.e., non-isometric and partial). This highlights the generalization and flexibility of the framework; see Figure \ref{fig:teaser} for an example. We introduce further losses that open to new families of bases\simone{.}
%, giving new tools to highlight the relationship between matching and function representation. 
We consider our discoveries surprising and counterintuitive, pointing to novel research directions in the field.

\rick{To summarize, our work presents the following novelties and contributions:}
\begin{enumerate}
    \item \emph{Extending the representation learned in \cite{LIE2020} to meshes, overtaking both LBO and \cite{LIE2020} in several settings}. To our best knowledge, this is the first study that presents a basis set that can better represent shape correspondence than LBO eigenfunctions, even for the near-isometric case.
    \item \emph{Offering an extensive analysis of the learned embedding}. While LBO has a long tradition, it is an original field for learned functional bases that deserve analyses and investigations. Our work highlights some misconceptions in the community and points to promising new directions.
    \item \rickn{\emph{Suggesting novel regularizations for the learned embeddings}. Starting from a theoretical ground, we formulate energies for training, shedding new light on two prominent properties (smoothness and orthogonality) that characterized the popularity of the LBO.}  
    
    % \item Involving learned embedding in the function representation task, exploring different kinds of losses; such application for learned embedding has never been addressed before, and we propose it as a fundamental tool to explore the properties of the obtained basis set.

\end{enumerate}

All the data and code will be made publicly available for research purposes.




==> sections/results.tex <==
\section{Results and analysis}
\label{sec:results}

\begin{figure*}[!t]
	%\centering
	\vspace{0.5cm}
	
	\footnotesize

    \begin{tabular}{c}
    \hspace{0.7cm}	
	\begin{minipage}{\linewidth}
	


		    
	\begin{overpic}[trim=0cm 0cm 0cm 0cm,clip, width=0.92\linewidth]{./figures/basis_2rows_cb_low.png}
		\put(-3,22){\scriptsize $\OurBasis$}
		\put(-3,10){\scriptsize $\LBOBasis$}
		\put(-7.6,30.6){\scriptsize $E_{D}(\OurBasis)$}
		\put(2,33.5){\scriptsize{$0.62$}}
		\put(12,33.5){\scriptsize{$1.18$}}
		\put(20,33.5){\scriptsize{ $1.94$}}
		\put(30,33.5){\scriptsize{$3.02$}}
		
		\put(43,33.5){\scriptsize{$9.63$}}
		\put(56,33.5){\scriptsize{$19.27$}}
		
		\put(71,33.5){\scriptsize{$90.97$}}
		\put(81,33.5){\scriptsize{$145.51$}}
		\put(91,33.5){\scriptsize{$160.99$} }  
		
		
		
		\put(39,10){{\dots} }  
		\put(38,25){{\dots} }  
		\put(53,10){{\dots} }  
		\put(52,25){{\dots} }  
		\put(65,10){{\dots} }  
		\put(65,25){{\dots} }  

        \put(98,11.95){{\tiny{$-\sigma$}} } 
        \put(98,14.4){\tiny{$0$} }
        \put(98,16.95){\tiny{$+\sigma$} } 
        
        \put(-7.6,0.3){\scriptsize{$E_{D}(\LBOBasis)$}}
		\put(3,-0.5){\scriptsize{$0$}}
		\put(12,-0.5){\scriptsize{$2.58$}}
		\put(20,-0.5){\scriptsize{$3.44$}}
		\put(30,-0.5){\scriptsize{$5.04$}}
		
		\put(43,-0.5){\scriptsize{$87.84$}}
		
		\put(56,-0.5){\scriptsize{$156.95$}}
		
		\put(71,-0.5){\scriptsize{$221.27$}}
		\put(81,-0.5){\scriptsize{$226.18$}}
		\put(91,-0.5){\scriptsize{$239.27$}}
		
		\put(3,-4.1){\scriptsize{$\mathbf{1^{th}}$}}
		\put(12,-4.1){\scriptsize{$\mathbf{2^{nd}}$}}
		\put(22,-4.1){\scriptsize{$\mathbf{3^{rd}}$}}
		\put(32,-4.1){\scriptsize{$\mathbf{4^{th}}$}}
		\put(45,-4.1){\scriptsize{$\mathbf{18^{th}}$}}
		\put(58,-4.1){\scriptsize{$\mathbf{28^{th}}$}}
		\put(73,-4.1){\scriptsize{$\mathbf{38^{th}}$}}
		\put(83,-4.1){\scriptsize{$\mathbf{39^{th}}$}}
		\put(93,-4.1){\scriptsize{$\mathbf{40^{th}}$}}
	\end{overpic}
	\vspace{0.3cm}
	
	\end{minipage}
    \end{tabular}
	\caption{We visualize the dimensions of the embeddings as function over the surface. For each one, we report its Dirichlet energy as a measure of the smoothness
	}
	\label{fig:basis}	
	%\hspace{-0.8cm}
\end{figure*}


\paragraph{Basis dimension.} For each one of $S+F$ and $F+S$, we train $5$ embedding networks with a different number of output dimensions (i.e., $5$,$10$,$20$,$30$, and $40$). On the test dataset, we computed the optimal matching between the $50$ pairs using the ground truth correspondence as described above:
\begin{align}
    C^{opt}_{\N\M} = \Phi_{\mathcal{M}}^\dagger  \Pi_{\mathcal{M}\mathcal{N}} \Phi_{\mathcal{N}}  \\    \Pi_{\mathcal{M}\mathcal{N}} = NN(\Phi_{\mathcal{M}} C^{opt}, \Phi_{\mathcal{N}}).
\end{align}
Even using the ground truth $\Pi_{\mathcal{M}\mathcal{N}}$ to compute $C^{opt}$, the bases may present some deformations which are not linearly alignable, and we measure exactly the error generated by this loss of information.

\paragraph{Properties of the learned basis.} We further studied what are the properties that make our embedding well-suited for shape matching. First, our embedding is always full rank, despite our basis not being orthogonal (unlike the LBO basis, which is orthogonal by construction). 
A second property worth investigating is smoothness.  LBO eigenfunctions form the smoothest orthonormal basis as measured by the Dirichlet energy, which in the discrete case reads for a basis vector $\Phi_i$:
\begin{equation}
    E_{D}(\Phi_i) = (\Phi_i / \|\Phi_i\|_2 )^T \Delta (\Phi_i / \|\Phi_i\|_2 )\,. 
\end{equation}
In Figure \ref{fig:basis}, we depict the embedding dimensions as functions over the surfaces and report the Dirichlet energy for each. Our embedding is significantly smoother than LBO one; this is possible since we do not impose orthogonality.

The results are reported in Table \ref{fig:opt}. 
The first observation is that increasing the embedding size has a positive effect, while a saturation occurs for both $\OurBasis$ and $\LBOBasis$. Secondly, we can compress the LBO representation in significantly smaller space (i.e., with $5$ learned dimensions, we have the same quality of $20$ LBO basis, with $10$ learned the same of $30$). But finally, and most importantly, our basis always produces a better matching w.r.t. LBO basis.  On the right of Table \ref{fig:opt}, we also depict the error of the two basis sets. With small bases, the $\LBOBasis$ cannot distinguish between the back and front of the shape, and at higher dimensions, the error peak at the protrusions. Learned embedding distributes the error more homogeneously over the surface.

\paragraph{Different Embeddings.} We report in Table \ref{tab:losses} the results with the ground truth transformation $C_{gt}$ for embeddings trained with the losses presented in Section \ref{sec:method}. As expected, the embedding learned with the supervised loss performs better. However, in our setting $L_{L1+S}$ preserves some matching capacity in F+S setting, highlighting interesting relations between linearly-invariant embeddings and general properties. Finally, \cite{LIE2020} shows that not only it cannot overtake LBO, but that $L_{L1+S}$ cannot be adopted. 
%This limitation of \cite{LIE2020} will be further shown in Section \ref{sec:func}.

\rickn{\paragraph{Different Regularizations.} We decided to explore the opportunities of our embedding by including different regularzations during the training. We report in Table \ref{tab:losses_reg} the results. First of all, we noticed that promoting the smoothness produce a slight improvement or keep stable results. This is expected from the above analysis, since the network already discover smoothness as a good property for the matching. Including $\Lo$ instead, is disruptive. By our investigation, we attribute the cause to the magnitude of this energy, that strongly bound the network to favor the bijctivity prior  over good matching. This motivated us to scale the energy to a magnitude similar to $\Ls$. At this point, the network obtained a significant gain. SMAL is the only dataset where smoothness seems slightly dangerous. We attribute this behavior the self-intersections and artifacts present on the muzzle of animals.
}

\begin{table}
\centering
	
	\begin{tabular}{@{}lrrr@{}}
		&  S+F    & F+S    & SMAL                  \\
		\hline
		$\OurBasis$      &  \textbf{1.58}    &  \textbf{1.52} & \textbf{1.8}  \\
		$L_{L1+E_D}$             &  13.18    &  5.72  & 14.9  \\
		%$L_{Coord}$            &  34.23   & 48.86     \\	
		LBO                    &   2.05   &  1.97 & 4.3 \\
		L-Invariant            &   2.94   &   2.85 & 2.4 \\
		%L-Invariant $L_{L1+S}$ & 66.34   &   81.01 
	\end{tabular}
	\caption{\label{tab:losses}
	Quantitative comparison on shape matching, learning a $40$ dimensional embedding, and computing the ground truth transformation $C_{opt}$. Each row is a different training.}
		%Quantitative comparison on the shape matching task.}
\end{table}

\begin{table}
\centering
	\begin{tabular}{@{}lrrr@{}}
		&  S+F    & F+S    & SMAL                  \\
		\hline
		$\OurBasis$      &  1.58    &  1.52 & 1.8 \\
		$\OurBasis_{+L_{E_D}}$          & 1.29 & \textbf{1.34}  & 2.0 \\
		$\OurBasis_{+\Lo}$       & 15.35 & 23.10 & 19.0 \\
		$\OurBasis_{+\Low}$  &  \textbf{1.19} & 1.41 & \textbf{1.4}\\
		$\OurBasis_{+L_{E_D}+\Low}$ & \textbf{1.19} & \textbf{1.35} & 5.9\\
	\end{tabular}
	\caption{\label{tab:losses_reg}
	Quantitative comparison on different regularizations, learning a $40$ dimensional embedding, and computing the ground truth transformation $C_{opt}$. Each row is a different training.}
\end{table}

\paragraph{Rotation invariance}
In shape matching, the rotation invariance is a desirable property. Our data augmentation is an effective technique to build resilience to rotations, without giving up extrinsic information. 
\setlength{\columnsep}{5pt}
\begin{wraptable}[5]{R}{0.2\linewidth}
	\footnotesize
	\vspace{-0.5cm}
    
    \begin{center}	    	
	\hspace{-1cm}

	\begin{tabular}{lr}
                            &  F+S \\ \hline
		$\OurBasis_{coord}$ &  \textbf{1.58}  \\
		$\OurBasis_{HKS}$   &  1.81   \\ \hline
		$\LBOBasis$         &  2.05   \\ 


	\end{tabular}
    \end{center}
    \vspace{-0.5cm}

	%\caption{\label{tab:HKS} \textit{Matching results on F+S.}}
\end{wraptable}

To clarify this, we considered a pair of test shapes in the F+S setting. We fixed one of the two, applying to the second 50 different random 3D rotations. The error without rotations is $2.43$; while the mean error after the $50$ rotations is $2.52$ with standard deviation (std) $0.11$. Moreover, in the inset table, we input $50$ scales of HKS (a rotation invariant descriptor) to train $40$ basis functions as done in \cite{sharp2020diffusion}.
$\OurBasis_{HKS}$ is better than LBO, but not better than our basis $\OurBasis_{coord}$ trained on coordinates.

\paragraph{Non-bijective cases.} \rickn{Given the previous results, we decide to verify our intuitions considering contexts where data are not in bijectivity. Differently from previous works (that considered remeshed dataset but with similar density), we consider configurations with a significant change in their number of vertices. In Table \ref{tab:nonbj} we learned and tested on different scenarios. The smoothness does not change or harm the performances. Adding orthogonality confirms our hypotesis: promoting bijectivity when this is not present worsen the results. Finally, the last column witness also that even when training and testing data are not in bijection it is dangerous for the network. Later, we will interpretate this result.}
\begin{table}
\centering
	
	\begin{tabular}{@{}lrrrrr@{}}
		&  $\Snob$+F  &  $\Snob$+$\Fnob$    & $\Fnob$+S & $\Fnob$+$\Snob$   & \test{S+F}        \\
		\hline
		$\LBOBasis$&                               2.05 & 1.88 & 1.97 & 2.04 & 2.05\\
		$\OurBasis$&               1.12 & \textbf{0.76} & \textbf{1.24} & \textbf{1.27} & \textbf{1.07}\\
		$\OurBasis_{+\Ls}$&         \textbf{1.10} & \textbf{0.77} & \textbf{1.23} & \textbf{1.27} & \textbf{1.07}\\
		$\OurBasis_{+\Low}$& 1.60 & 1.61 & 1.50 & 1.55 & 1.14  \\
		$\OurBasis_{+\Ls+\Low}$ & 1.77 & 1.76 & 1.58 & 1.61 & 1.19

	\end{tabular}
	\caption{\label{tab:nonbj}
	Quantitative comparison on shape matching, learning a $40$ dimensional embedding, and computing the ground truth transformation $C_{opt}$. Each row is a different training.}
		%Quantitative comparison on the shape matching task.}
\end{table}

\vspace{0.25cm}


\section{Applicative scenarios}
% Many previous works that we discussed in Section \ref{sec:related} validate their matching performance on the S+F and F+S settings. We report in the Supplementary Material the results of our approach learning also the descriptors on them. Here we focus on more exciting challenges: non-isometric shapes, in which the considered objects may have a significant difference in their surface metric; and partiality, where at least the source shape has a missing component. The community has pushed the LBO to tackle both cases, working with ad-hoc refinement techniques, regularization, or new descriptors. We show learned embeddings are relisient and flexible in these contexts.
\rickn{While our analysis mainly focus on theoretical properties of learned embedding, we would emphasize some contexts in which they show also a significant applicability. Not only we are able to learn descriptors that significantly overtake state-of-the-art results, but also obtain better performance then the \emph{theoretically best possible results with LBO}. Further preliminar evidence on descriptor learning, matching refinement, and functional reconstruction can be found in Supplementary Material. 
\paragraph{Learning descriptors}
Many previous works that we discussed in Section \ref{sec:related} validate their matching performance on the S+F and F+S settings. We report in the Supplementary Material the results of our approach learning also the descriptors on them. Here we focus on more exciting challenges: non-isometric shapes, in which the considered objects may have a significant difference in their surface metric. In the table of Figure \ref{fig:tosca}, we report the results. First of all, we notice that good descriptors can be recovered even for our embedding without any further regularization. Once again, we observe also that smoothness is not particularly favorable in this context. Finally, the most exciting result is given by $Our^{\EmbNet}_{+\Low}$, that exhibit performance better then the best possible achievable by LBO (that is 4.3, from Table \ref{tab:losses}).
}

\begin{figure*}[!t]
\begin{tabular}{cc}
\begin{minipage}{0.26\linewidth}
    \footnotesize
	\begin{tabular}{@{}lr@{}}
		          & SMAL          \\
		\hline
		$Our^{\EmbNet}$                & 5.67 \\
		$Our^{\EmbNet}_{+\Ls}$         &   11.0   \\
		$Our^{\EmbNet}_{+\Low}$         &  \textbf{3.9}    \\
		$Our^{\EmbNet}_{+\Ls+\Low}$         &   11.5   \\ \hline
		$\DiffNet$         &  7.94               \\
		Universal          &  5.91      \\
		L-Invariant \cite{LIE2020} &	21.10 \\
        $GFM_{KP}$ \cite{donati2020deep} &     8.00 \\ 
        Deep Shells \cite{eisenberger2020deep}	& 15.23

	\end{tabular}
	\vspace{-0.2cm}
	
\end{minipage}
&

\begin{minipage}{0.7\linewidth}
	\scriptsize
	\vspace{0.2cm}
	\begin{overpic}[trim=0cm 0cm 0cm 0cm,clip, width=1.04\linewidth]{./figures/wolf_dog_lie.png}
		\put(8,-2.5){$\M$}
		\put(27,-2.5){Our}
		\put(44,-2.5){$GFM_{DN}$}
		\put(48,-6.0){\cite{donati2020deep}}
		\put(64,-2.5){Universal}
		\put(82,-2.5){L-Invariant} \put(87.5,-6.0){\cite{LIE2020}}
	\end{overpic}
	\vspace{-0.3cm}
	

\hspace{-0.2cm}
\end{minipage}

\end{tabular}

	\caption{\label{fig:tosca} On the left, a quantitative comparison on non-isometric shape matching on SMAL dataset. On the right, a pair of animals from TOSCA \cite{TOSCA} dataset, showing our generalization capability.}
\end{figure*}
\paragraph{Basis refinement (ZoomOut).} In recent years, several methods have relied on refining the matching using ZoomOut \cite{melzi2019zoomout}. This is a significantly important aspect for real case applications, and it may seem a drawback of learned embedding of which dimension must be decided at training time. However, thanks to their smoothness, the learned basis can be augmented as well by ZoomOut, refining the matching by including the LBO eigenfunctions at increasing frequencies. Given the limited space and the different focus of our narration, we report in the Supplementary Material the evidence of this possibility, showing that $\OurBasis$ can be combined with $\LBOBasis$. To our best knowledge, no other studies analyze ZoomOut refinement on different bases from $\LBOBasis$.


		



